Multi-Winner Election Control via Social Influence

In an election, we are given a set of voters, each having a preference list over a set of candidates, that are distributed on a social network. We consider a scenario where voters may change their preference lists as a consequence of the messages received by their neighbors in a social network. Specifically, we consider a political campaign that spreads messages in a social network in support or against a given candidate and the spreading follows a dynamic model for information diffusion. When a message reaches a voter, this latter changes its preference list according to an update rule. The election control problem asks to find a bounded set of nodes to be the starter of a political campaign in support (constructive problem) or against (destructive problem) a given target candidate $c$, in such a way that the margin of victory of $c$ w.r.t. its most voted opponents is maximized. It has been shown that several variants of the problem can be solved within a constant factor approximation of the optimum, which shows that controlling elections by means of social networks is doable and constitutes a real problem for modern democracies. Most of the literature, however, focuses on the case of single-winner elections. In this paper, we define the election control problem in social networks for "multi-winner elections" with the aim of modeling parliamentarian elections. Differently from the single-winner case, we show that the multi-winner election control problem is NP-hard to approximate within any factor in both constructive and destructive cases. We then study a relaxation of the problem where votes are aggregated on the basis of parties (instead of single candidates), which is a variation of the so-called "straight-party voting" used in some real parliamentarian elections. We show that the latter problem remains NP-hard but can be approximated within a constant factor.

==> trunk/MultiMessage.tex <==
\section{Multi-Message Model}
In this part, we consider the situation that a node can send several messages. The messages can be either constructive or destructive for our target party or an opponent party, respectively.
Each message $m$ can target just one party and influence whole candidates of the party. 
Then we define message $m = (m_1, m_2, \dots, m_{|C|}), \mbox{ s.t. } \exists m_i \in \{-1, 1\}, \forall m_j \neq m_i, m_j = 0$; in other words, the message contains either positive or negative information for exactly one party.
In this mode, the diffusion proceed the same as before for any message.

==> trunk/SingleWinner.tex <==
\section{Single-Winner Election Control Using General Scoring Rule}
\label{sec:singleWinnerGeneralScoringRule}
Let us consider the single-winner election control akin Wilder and Vorobeychik~\cite{wilder2018controlling} using non-increasing scoring function $f(\cdot)$, we name this problem \SWGS.
%In the following, we show that 
Since this problem is a more general version of the single-winner election control using the plurality scoring rule, then it is an $\NP$-hard problem.
In the following, we present an approximation algorithm for this problem.
%\todo{Revise this part to shrink it as much as possible. May we do not need of the definitions and so on.}
%In this case, there is no party, $C$ is a set of candidates, and the target candidate is $\cstar \in C$.
%We consider $\pi_v(c), \tilde{\pi}_v(c)$, respectively, as the preferences list of node $v$ before and after a diffusion process. 
%The activated nodes after $S$, promote (resp. demote) the rank of the target candidate by one on the constructive (resp. destructive) model.

%More formally, in the constructive case, for all nods $v \in A_S$, if $\pi_v(\cstar) > 1$, then $\tilde{\pi}_v(\cstar) = \pi_v(\cstar) -1$, and for the candidate $c \in C$ s.t. $\pi_v(c) = \pi_v(\cstar) -1$ we have $\tilde{\pi}_v(c) = \pi_v(c) +1$;
%also, for all other candidates $c_1 \in C$ s.t. $c_1 \neq c$ their rank will remain the same as before, i.e., $\tilde{\pi}_v(c_1) = \pi_v(c_1)$.
%For the destructive model, for all nods $v \in A_S$, if $\pi_v(\cstar) < |C|$, then $\tilde{\pi}_v(\cstar) = \pi_v(\cstar) + 1$, and for the candidate $c \in C$ s.t. $\pi_v(c) = \pi_v(\cstar) + 1$ we have $\tilde{\pi}_v(c) = \pi_v(c) - 1$;
%also, for all other candidates $c_1 \in C$ s.t. $c_1 \neq c$ their rank will remain the same as before, i.e., $\tilde{\pi}_v(c_1) = \pi_v(c_1)$.
%Note that for all non-active nodes $v \in V \setminus A_S$, in both constructive and destructive, the preferences list of $v$ does not change, i.e., $\tilde{\pi}_v = \pi_v$.


% Let us define the non-increasing scoring function $f : \{1, 2, \dots, |C| \} \rightarrow \R_{\geq 0}$ which assigns a non-negative real number to each rank as the score of the rank. 
The scoring function $f(\cdot)$ is the same as before (see Section~\ref{subsec:objectiveFunction}).
Also, the score of a candidate $c$ before and after $S$, respectively, is presented as $\F(c, \emptyset) = \sum_{v \in V} f(\pi_v(c))$ and $\F(c, S) = \E \big[ \sum_{v \in V} f(\tilde{\pi}_v(c)) \big]$.
%Let us consider $\cmoa{S}, \cmob$ as the most voted opponent candidates before and after $S$, respectively.
We define \textit{Margin of Victory - MoV}, the same as Wilder and Vorobeychik~\cite{wilder2018controlling}.%, for a target candidate $\cstar \in C$, in both constructive and destructive cases.% as follows.
% \begin{align*}
%     \MOV(\cstar, S) &= \F(\cstar, S) - \F(\cmoa{S}, S) - \\ & \quad
%     \left( \F(\cstar, \emptyset) - \F(\cmob, \emptyset) \right),\\
%     \MOVD(\cstar, S) &= \F(\cstar, \emptyset) - \F(\cmob, \emptyset) - \\ & \quad 
%     \left( \F(\cstar, S) - \F(\cmoa{S}, S) \right).
% \end{align*}
Also, we define \textit{Difference of Votes - DoV} for the target candidate $\cstar$, in both constructive and destructive cases as %follows.
%\begin{align*}
    $\DOVP(\cstar, S) = \F(\cstar, S) - \F(\cstar, \emptyset)$, and 
    $\DOVDN(\cstar, S) = \F(\cstar, \emptyset) - \F(\cstar, S)$.
%\end{align*}
% Note that DoV for other candidates $c \in C, c \neq \cstar$ is defined as follows.
% \begin{align*}
%     \DOVN(c, S) &= \F(c, \emptyset) - \F(c, S),\\
%     \DOVDP(c, S) &= \F(c, S) - \F(c, \emptyset).
% \end{align*}

\iffalse
\begin{thrm}
It is $\NP$-hard to maximizing $\MOV$ (respectively, $\MOVD$) and $\DOV$ (respectively, $\DOVD$)
for \SWGS.
\end{thrm}

\begin{proof}
\todo{As it is a more general version of plurality, is it necessary to reduce from plurality to the general scoring rule?}
\end{proof}
\fi

% The diffusion of a set of seed nodes $S$ in ICM is equal to the reachable nodes from the same seed set in a set of random graphs, called live-edge graph~\cite{kempe2015maximizing}.
% Given $G(V, E)$ as a graph for ICM, to create a live-edge graph $G'(V', E')$, we do as follows.
% The $G'$ contains the same nodes and edges of $G$, i.e., $V' = V, E' = E$.
% Afterwards, for each edge $(u, v) \in E'$ with weight $0 \leq b_{uv} \leq 1$, %we add the edge to the $E'$ with probability $b_{uv}$, i.e., 
% we remove $(u, v)$ from $E'$ with probability $1 - b_{u,v}$. 
% At the end, we set the weight of all edges $(u, v) \in E'$ equal to 1.
% Let us denote by $\G$ the set of all possible live-edge graphs that can be generated from $G$.
% Also, let us define $R(g, S)$ as the set of nodes in $g \in \G$ reachable from the set of seed nodes $S$.
% Note that finding a set of seed nodes to maximize the diffusion under the live-edge model is sub-modular~\cite{kempe2015maximizing}.

In the following lemma, we show that by using the standard greedy algorithm~\cite{kempe2015maximizing}, we can get a $(1- \frac{1}{e})$-approximation factor for $\DOV$ (respectively, $\DOVD$).
After that, we proof that by maximizing $\DOV$ (respectively, $\DOVD$), we get a constant factor approximation for maximizing $\MOV$ (respectively, $\MOVD$).

Since this version is a careful extension of the single-winner election control using plurality scoring rule~\cite{wilder2018controlling}, and also due to the space limitation we omitted the proofs.
Note that we can assign a weight to each node which is equal to the difference score of the target candidate if the node become active, 
and the problem will be reduced to the IM problem.
%\todo{Mention here that the analysis is very similar to the Wilder and vob..., and due to space limitation and similarity we omitted the proof.}

\begin{lemma}
\label{lemma:SingleWinnerDOVApproximationFactor}
Using the standard greedy algorithm for influence maximization problem provides $(1-\frac{1}{e})$-approximation factor to maximize $\DOV$ (respectively,  $\DOVD$) in \SWGS.
\end{lemma}

\iffalse
\begin{proof}
\todo{Removed due to the space limitation.}
First, we consider the constructive model, i.e., $\DOV$. 
In this model, the nodes that before any diffusion prefer $\cstar$ the most, will not change the score of $\cstar$ after diffusion (even though they may activate other nodes). 
On the other hand, all of the nodes that do not prefer $\cstar$ to all other candidates can increase the score of $\cstar$ by $f(\pi_v(\cstar)-1) - f(\pi_v(\cstar))$\footnote{We assume function $f(\cdot)$ is defined in such away that $f(\pi_v(\cstar)-1) - f(\pi_v(\cstar))$ is a constant number. In other words, $f(\pi_v(\cstar)-1) - f(\pi_v(\cstar))$ does not depend on $|V|$. This is important because influence maximization problem is still an open problem when $f(\pi_v(\cstar)-1) - f(\pi_v(\cstar))$ depends on number of nodes in the graph~\cite{kempe2015maximizing}.}.
By this observation, we assign weight 0 to the nodes that prefer $\cstar$ the most, and $f(\pi_v(\cstar)-1) - f(\pi_v(\cstar))$ to the nodes $v \in \{ u \in V| \pi_u(\cstar) > 1 \}$. 
Then the standard greedy algorithm, presented by Kempe et al.~\cite{kempe2015maximizing} for IM problem, guarantee a $(1-\frac{1}{e})$-approximation factor.

More precisely, let us define $S$ as the set of seed nodes returned by the algorithm and $A_S$ as the activated nodes after $S$. 
Also, $S^*$ and $A_{S^*}$ are the optimal seed set, and corresponding activated nodes for the problem, respectively.
Then we have
\begin{align*}
    &\DOV(\cstar, S) = \F(\cstar, S) - \F(\cstar, \emptyset)\\
    &= \E \big[ \sum_{v \in V} f(\tilde{\pi}_v(\cstar)) \big] - \sum_{v \in V} f(\pi_v(\cstar))\\ 
    &= \sum_{v \in V} \E \big[ f(\tilde{\pi}_v(\cstar)) \big] - \sum_{v \in V} f(\pi_v(\cstar))\\ 
    &= \sum_{v \in V: \pi_v(\cstar) = 1} f(1) \\ & \quad + \sum_{v \in V: \pi_v(\cstar)>1}  
    \E \big[ f(\tilde{\pi}_v(\cstar)) \big]- \sum_{v \in V} f(\pi_v(\cstar))\\ 
    &= \sum_{v \in V: \pi_v(\cstar) = 1} f(1) \\ & \quad + \sum_{v \in V: \pi_v(\cstar)>1} \big[ f(\pi_v(\cstar)-1)\Pr(v \in A_S) + \\ &\quad f(\pi_v(\cstar))(1-\Pr(v \in A_S)) \big] - \sum_{v \in V} f(\pi_v(\cstar))\\ 
    &= \sum_{v \in V: \pi_v(\cstar) = 1} f(1) + \sum_{v \in V: \pi_v(\cstar)>1} \Big[f(\pi_v(\cstar)) + \\ & \quad \Pr(v \in A_S) \left( f(\pi_v(\cstar)-1))-f(\pi_v(\cstar)) \right) \Big] - \sum_{v \in V} f(\pi_v(\cstar))\\
    &= \sum_{v \in V} f(\pi_v(\cstar)) + \sum_{v \in V: \pi_v(\cstar)>1} \Big[ \Pr(v \in A_S) \big( f(\pi_v(\cstar)-1) -  \\ & \quad 
    f(\pi_v(\cstar)) \big) \Big] - \sum_{v \in V} f(\pi_v(\cstar))\\
    &= \sum_{v \in V: \pi_v(\cstar)>1} \Pr(v \in A_S) \left( f(\pi_v(\cstar)-1)-f(\pi_v(\cstar)) \right)\\
    &= \sum_{i = 2}^{|C|} (f(i-1)-f(i)) \sum_{v \in V: \pi_v(\cstar) = i} \Pr(v \in A_S)\\
    &= \sum_{i = 2}^{|C|} (f(i-1)-f(i)) \sum_{v \in V: \pi_v(\cstar) = i} \sum_{g \in \mathcal{G}} \mathds{1}_{v \in R(g, S)}\Pr(g)\\
    &= \sum_{i = 2}^{|C|} (f(i-1)-f(i)) \sum_{g \in \mathcal{G}}\Pr(g)\Big| R(g, S) \cap \{v \in V | \pi_v(\cstar) > 1\}\Big|
\end{align*}  
Since it is monotone and sub-modular~\cite{kempe2015maximizing}\todo{Check this to make sure that they have proofed this.}, then by using the greedy algorithm we get $(1- \frac{1}{e})$- approximation factor; then it yields
\begin{align*}
    \DOV(\cstar, S) &\geq (1- \frac{1}{e}) \sum_{i = 2}^{|C|} (f(i-1)-f(i))  \\ & 
    \sum_{g \in     \mathcal{G}}\Pr(g)\Big| R(g, S^*) \cap \{v \in V | \pi_v(\cstar) > 1\}\Big|\\
    &= (1- \frac{1}{e})\DOV(\cstar, S^*),
\end{align*}
and concludes the constructive model.
For destructive case, it is the same as constructive except that if the target candidate is the least preferred candidate in a preferences list of a node $v$, then $v$ cannot decrease the score of $\cstar$; otherwise, the score can be reduced by $f(\pi_v(\cstar))-f(\pi_v(\cstar)+1)$. 
The same approach yields the same approximation factor for $\DOVD$.
\todo{As the proof is similar to the constructive case, do we have to write it?}

\end{proof}
\fi

Using Lemma~\ref{lemma:SingleWinnerDOVApproximationFactor}, we present a constant factor approximation algorithm for $\MOV$ and $\MOVD$.

\begin{thrm}
\label{theorem:singleWinnerConstMOV}
Maximizing $\DOVP$ (resp. $\DOVDN$) obtains $\frac{1}{3}(1-\frac{1}{e})$ (resp. $\frac{1}{2}(1-\frac{1}{e})$)-approximation to the $\MOV$ (resp. $\MOVD$).
\end{thrm}


\iffalse
\begin{proof}


\begin{align*}
    &\MOV(\cstar, S) = \F(\cstar, S) - \F(\cmoa{S}, S) -
    \left( \F(\cstar, \emptyset) - \F(\cmob, \emptyset) \right)\\
    &= \DOVP(\cstar, S) + \DOVN(\cmoa{S}, S) - \F(\cmoa{S}, \emptyset) + \F(\cmob, \emptyset)\\
    &\geq (1- \frac{1}{e})\DOVP(\cstar, S^*) - \F(\cmoa{S}, \emptyset) + \F(\cmob, \emptyset)\\
    &\stackrel{(a)}{\geq} \frac{1}{3}(1- \frac{1}{e})\left[\DOVP(\cstar, S^*) + \DOVN(\cmoa{S^*}, S^*) + \DOVN(\cmoa{S}, S^*) \right] - \\ & \quad \quad \F(\cmoa{S}, \emptyset) + \F(\cmob, \emptyset)\\
    &\stackrel{(b)}{\geq} \frac{1}{3}(1- \frac{1}{e})\Big[\DOVP(\cstar, S^*) + \DOVN(\cmoa{S^*}, S^*) + \DOVN(\cmoa{S}, S^*) - \\ & \quad \quad \F(\cmoa{S}, \emptyset) + \F(\cmob, \emptyset) + \F(\cmoa{S^*}, \emptyset) - \F(\cmoa{S^*}, \emptyset) \Big]\\
    &= \frac{1}{3}(1- \frac{1}{e}) \Big[ \MOV(\cstar, S^*) + \DOVN(\cmoa{S}, S^*) \\ &\quad + \F(\cmoa{S^*}, \emptyset) - \F(\cmoa{S}, \emptyset) \Big]\\
    &\stackrel{(c)}{\geq} \frac{1}{3}(1- \frac{1}{e})\MOV(\cstar, S^*)
\end{align*}
Where the inequality $(a)$ holds because all of the scores lost by $\cmob$ and $\cmoa{S^*}$ will be added to the score of $\cstar$ by definition, and inequality $(b)$ is correct because $\F(\cmob, \emptyset) \geq \F(\cmoa{S}, \emptyset)$ by definition.
Also, the inequality $(c)$ holds because 
\begin{align*}
    &\DOVN(\cmoa{S^*}, S^*) - \DOVN(\cmoa{S}, S^*) \\
    &= F(\cmoa{S^*}, \emptyset) - F(\cmoa{S^*}, S^*) -  F(\cmoa{S}, \emptyset) + F(\cmoa{S}, S^*) \\
    &\stackrel{(d)}{\leq} F(\cmoa{S^*}, \emptyset) - F(\cmoa{S}, \emptyset)\\
    &\Rightarrow 0 \leq \DOVN(\cmoa{S^*}, S^*) \leq \\ &\quad  \DOVN(\cmoa{S}, S^*) + \F(\cmoa{S^*}, \emptyset) - \F(\cmoa{S}, \emptyset) 
\end{align*}
Where $(d)$ holds because $F(\cmoa{S}, S^*) \leq F(\cmoa{S^*}, S^*)$.


\end{proof}


\begin{thrm}
\label{theorem:singleWinnerDestMOV}
Maximizing $\DOVDN$ obtains $\frac{1}{2}(1-\frac{1}{e})$-approximation to the $\MOVD$.
\end{thrm}

\begin{proof}

\begin{align*}
    &\MOVD(\cstar, S) = \F(\cstar, \emptyset) - \F(\cmob, \emptyset) - %\\ & \quad 
    \left( \F(\cstar, S) - \F(\cmoa{S}, S) \right)\\
    &= \DOVN(\cstar, S) + \DOVP(\cmoa{S}, S) + \F(\cmoa{S}, \emptyset) - \F(\cmob, \emptyset)\\
    &\geq (1- \frac{1}{e})\DOVN(\cstar, S^*) + \DOVP(\cmoa{S}, S) + \F(\cmoa{S}, \emptyset) - \F(\cmob, \emptyset)\\
    &\stackrel{(a)}{\geq} \frac{1}{2}(1- \frac{1}{e})\left[\DOVN(\cstar, S^*) + \DOVP(\cmoa{S^*}, S^*) \right] + \DOVP(\cmoa{S}, S) + \\ & \quad \quad \F(\cmoa{S}, \emptyset) - \F(\cmob, \emptyset)\\
    &\stackrel{(b)}{\geq} \frac{1}{2}(1- \frac{1}{e})\Big[\DOVN(\cstar, S^*) + \DOVP(\cmoa{S^*}, S^*) + \DOVP(\cmoa{S}, S) + \\ & \quad \quad \F(\cmoa{S}, \emptyset) - \F(\cmob, \emptyset) + \F(\cmoa{S^*}, \emptyset) - \F(\cmoa{S^*}, \emptyset)\Big]\\
    &= \frac{1}{2}(1- \frac{1}{e}) \Big[ \MOVD(\cstar, S^*) + \DOVP(\cmoa{S}, S) - \F(\cmoa{S^*}, \emptyset) + \F(\cmoa{S}, \emptyset) \Big]\\
    &\stackrel{(c)}{\geq} \frac{1}{2}(1- \frac{1}{e})\MOVD(\cstar, S^*)
\end{align*}
Where the inequality $(a)$ holds because $\cmoa{S^*}$ can gain at most all of the scores lost by $\cstar$.
For inequality $(b)$ we have
\begin{align*}
    & \DOVP(\cmoa{S}, S) + \F(\cmoa{S}, \emptyset) - \F(\cmob, \emptyset) \\
    =& \F(\cmoa{S}, S) - \F(\cmoa{S}, \emptyset) + \F(\cmoa{S}, \emptyset) - \F(\cmob, \emptyset) \\
    =& \F(\cmoa{S}, S)  - \F(\cmob, \emptyset),
\end{align*}
and by definition $\F(\cmoa{S}, S) \geq \F(\cmob, \emptyset)$.
Also, the inequality $(c)$ is correct because 
\begin{align*}
     &\DOVP(\cmoa{S}, S) - \F(\cmoa{S^*}, \emptyset) + \F(\cmoa{S}, \emptyset) \\
     =& \F(\cmoa{S}, S) - \F(\cmoa{S}, \emptyset) - \F(\cmoa{S^*}, \emptyset) + \F(\cmoa{S}, \emptyset)\\
     =& \F(\cmoa{S}, S) - \F(\cmoa{S^*}, \emptyset)
\end{align*}
and by definition $\F(\cmoa{S}, S) \geq \F(\cmoa{S^*}, \emptyset)$.

\end{proof}

\fi

==> trunk/alg-greedy.tex <==
\begin{algorithm}[t]
\caption{\textsc{Greedy}}\label{alg:1-playerAlg}
\begin{algorithmic}[1]
\Require{Social graph $G=(V,E)$; Budget $B$}
\State $\hat{G} = (G, w)$  \Comment{Weighted graph $\hat{G}$}
\State $S = \emptyset$
\While{$|S| \leq B$}
% \State $v = \argmax_{u \in V \setminus S} F(\cstar, S \cup \{u\}) - F(\cstar, S)$ \label{alg:row-argmax}\federico{?}
\State $v = \argmax_{u \in V \setminus S} \sigma_w(S \cup \{u\}) - \sigma_w(S)$
\State $S = S \cup \{ v \}$
\EndWhile
\State \Return{$S$}
\end{algorithmic}
\end{algorithm}

==> trunk/background.tex <==
\section{Background}
\label{sec:background}
%In this part, we introduce three essential notions as follows. 

%\paragraph{Voting Systems.}
%\subsection{Voting Systems}
%\label{subsec:votingSystems}
%In this part, we consider the rules that are used in the election, known as \emph{voting systems}.
% Since \emph{computational social choice}, is a field at the intersection of social choice theory, theoretical computer science, and multi-agent systems' analysis, then it contains a very different variety of problems from \textit{voting theory} and \textit{fair allocation}~\cite{brandt2016handbook}.
% In particular, this problem consists of the analysis of the computational complexity of computing the result of voting rules. It can also be considered as a barrier against strategic manipulation in elections~\cite{brandt2016handbook,chevaleyre2007short,endriss2017trends,faliszewski2010ai}.
We focus \emph{multi-winner} voting systems, where the $k$ candidates with the highest score are elected. These voting system is commonly used in real-world elections, like parliamentarian elections. Each voter has a preference list over the candidates and a score is assigned to each candidate according to a non-increasing scoring function of the lists. Non-increasing scoring rules generalize many well known scoring rules, such as, plurality, $t$-approval, Borda's rule, veto (anti-plurality).


%\paragraph{Influence Maximization.}
%\subsection{Influence Maximization}
%\label{subsec:influenceMaximization}

\textit{Influence maximization} is the problem of finding a small subset of nodes (as seed nodes) in a social network in order to maximize the spread of influence.
In this work, we use the \textit{Independent Cascade Model} (ICM), a well-known model for influence maximization introduce by Kempe et al. ~\cite{kempe2015maximizing}.
In this model, each edge $(u, v) \in E$ has a weight $b_{uv} \in [0, 1]$.
The influence will start with a set of seed nodes $S$ and keep activating the nodes in at most $|V|$ discrete steps.
In the first step, all the seed nodes $S$ become active. In the next steps $i>1$, all the nodes that were active in step $i-1$ remain active, moreover, nodes that became active at step $i-1$ try to activate their outgoing neighbors at step $i$ as follows.
When node $u$ becomes active at step $i-1$, it activates each of its neighbors $v \in \Nout{u}$ with probability  $b_{uv}$. Each active node will try to activate its outgoing neighbors independently and only once.
This process stops when no new node becomes active. We define $A_S$ as a set of nodes that are eventually active by the diffusion started by the seeds $S$.



%\paragraph{Election Control.}
%\subsection{Election Control}
%\label{subsec:electionControl}

%The \textit{election control} refers to the influence maximization problem when a political campaign targets a social network of voters; it can be done to handle the result of the election, i.e., to either ensure that a target candidate wins (constructive), or loses (destructive).

% Wilder and Vorobeychik studied this problem under ICM in the single-winner model. 
% They provide some positive and negative results for maximizing the, respectively, \emph{Margin of Victory} (MoV) and \emph{Probability of Victory} of a target candidate concerning the most voted opponent.
% In their model, the adversary wants to change the outcome of the election by spreading messages.
% It causes voters to change their preferences over the candidates. In constructive mode, the adversary can spread a message which causes to promote $\cstar$ by one place in the preferences list of the activated nodes. 
% In an active node $v$, if the target candidate $\cstar$ is already the most preferred candidate, then the message does not affect $v$, but $v$ can still share the message with its neighbors. In destructive control, a voter who is influenced demotes $\cstar$ by one place~\cite{wilder2018controlling}.
% Later, in Section~\ref{sec:straightParty}, we refer to this model by \textit{original model} (OM).

